How Compression and Approximation Affect Efficiency in String Distance Measures

Real-world data often comes in compressed form. Analyzing compressed data directly (without decompressing it) can save space and time by orders of magnitude. In this work, we focus on fundamental sequence comparison problems and try to quantify the gain in time complexity when the underlying data is highly compressible. We consider grammar compression, which unifies many practically relevant compression schemes. For two strings of total length $N$ and total compressed size $n$, it is known that the edit distance and a longest common subsequence (LCS) can be computed exactly in time $\tilde{O}(nN)$, as opposed to $O(N^2)$ for the uncompressed setting. Many applications need to align multiple sequences simultaneously, and the fastest known exact algorithms for median edit distance and LCS of $k$ strings run in $O(N^k)$ time. This naturally raises the question of whether compression can help to reduce the running time significantly for $k \geq 3$, perhaps to $O(N^{k/2}n^{k/2})$ or $O(Nn^{k-1})$. Unfortunately, we show lower bounds that rule out any improvement beyond $\Omega(N^{k-1}n)$ time for any of these problems assuming the Strong Exponential Time Hypothesis. At the same time, we show that approximation and compression together can be surprisingly effective. We develop an $\tilde{O}(N^{k/2}n^{k/2})$-time FPTAS for the median edit distance of $k$ sequences. In comparison, no $O(N^{k-\Omega(1)})$-time PTAS is known for the median edit distance problem in the uncompressed setting. For two strings, we get an $\tilde{O}(N^{2/3}n^{4/3})$-time FPTAS for both edit distance and LCS. In contrast, for uncompressed strings, there is not even a subquadratic algorithm for LCS that has less than a polynomial gap in the approximation factor. Building on the insight from our approximation algorithms, we also obtain results for many distance measures including the edit, Hamming, and shift distances.

==> SummaryCompressedApproximate.tex <==
\subsubsection*{Compressed Approximate Median Edit Distance}

For the (median) edit distance between $k$ strings, we show that allowing $(1+\epsilon)$-approximation gives an algorithm circumventing the bound in Theorem~\ref{thm:editDistanceLowerBoundFromSETH}:

\begin{theorem}\label{thm:k-ed}
    Given $k=\Oh(1)$ straight-line programs $\G_{X_i}$ of total size $n$ generating strings $X_i$
    of total length $N>0$ and a parameter $\eps \in (0,1]$,
    an integer between $\ED(X_1,\ldots,X_k)$ and $(1+\eps)\ED(X_1,\ldots,X_k)$
    can be computed in $\Ohtilde\left(\eps^{-\Oh(k)}n^{k/2}N^{k/2}\right)$ time.
\end{theorem}

The proof is given in~\cref{sec:k-ed}. For the edit distance between $k$ compressible strings, we use a different set of techniques than in the two-string case. Most approaches for speeding up the textbook DP algorithm for two (compressible) strings, including the aforementioned results in this paper, rely on the ability to perform computations involving DIST matrices efficiently. These computations crucially depend on the fact that DIST matrices satisfy the Monge property. However, for the natural high-dimensional generalization of DIST matrices, we do not know of any analog of the Monge property they satisfy that allows us to perform similar computations even for three-string similarity problems. Indeed, most natural generalizations of the Monge property seem to break down even in the three-string setting (see~\cref{sec:disttensor} for more details). 
Thus, it appears unlikely that, for example, an algorithm that partitions the DP table into boxes and computes the DP values on the boundary of each box using computations involving DIST matrices would be substantially more efficient than the textbook edit-distance algorithm, even in the three-string setting.

While we may not be able to compute DIST matrices to efficiently query the distance between any two points on the boundary of a box in the DP table, we are able to compute the distance between the ``top-left'' and ``bottom-right'' corner of every box in the DP table efficiently if there are not too many different boxes.
However, if we naively were to partition strings to form boxes similarly to how we partition strings the two-string setting (where each phrase corresponds to an SLP symbol of an auxiliary grammar), it may be the case that no low-cost alignment comes close to the corners of the boxes in the DP table. 
In this case, knowing the distances between these corners is not sufficient for estimating the median edit distance. 

To get around this issue, we use the window-respecting alignment framework that has been of much recent interest in works on edit distance (see e.g.~\cite{BEGHS18,CDGKS18,GRS:20}).
At a high level, the window-respecting alignment partitions the first string $X_1$ into substrings of length $\tau$, which we call ``windows'', and then considers a set of windows in the remaining strings. Informally, for every string length $L$ such that $L$ equals $\tau$ plus or minus a power of $(1+\epsilon)$ and $L \leq \tau / \epsilon^2$, and for every starting position $P$ that is a multiple of $\frac{\epsilon \tau}{|X_1|} \cdot \ED(X_1, X_2, \ldots, X_k)$, we have a window that is the substring of length $L$ starting at position $P$.
Since these windows are a ``net'' of all substrings we might consider matching windows in $X_1$ with, we can show that there is a $(1+\epsilon)$-approximate alignment that matches each window in $X_1$ precisely to a window in every other string. 
Given this property, it does suffice to only compute the ``corner-to-corner'' distance for each block in the DP table corresponding to a tuple of windows, rather than the distance between all pairs of points on these blocks' boundaries. Furthermore, we can compute (a $(1+\epsilon)$-approximation of) the optimal window-respecting alignment efficiently using a DP algorithm running in time $\tilde{O}_\epsilon (N^k/\tau^k)$.

Now, to implement the DP naively, we would need to compute the edit distances for each of $\tilde{O}_\epsilon (N^k/\tau^k)$ $k$-tuples of windows in $\Oh(\tau^k)$ time each. To reduce the running time, we show the following simple but powerful property of compressible strings:
For any string $X$ generated by an SLP of size $n$, we can in $O(|X|)$ time identify a set of $O(n\tau/\delta)$ ``representative'' strings $S$ such that every substring of $X$ of length $\tau$ is within edit distance $\delta$ to one of these representative strings.
The strength of this property is that these representatives approximate all the length-$\tau$ substrings of $X$, not just those corresponding to a symbol in an auxiliary grammar.
Now, for all $d$ that are powers of 2, setting $\delta = \epsilon d$, we can compute the edit distance between all $k$-tuples of representative strings for which the edit distance is at most $d$ in time $\tilde{O}_\epsilon(n^k \tau^k)$, and this gives us a reasonably good approximation of the edit distances between all $k$-tuples of windows. Our final algorithm is now just to solve the DP for finding an optimal window-respecting alignment, using this approximation instead of the exact distances between $k$-tuples of windows, and the choice $\tau = \sqrt{N/n}$ gives the desired runtime.

\subsubsection*{Approximate Center Edit Distance for Many Strings}
Using a similar framework to our median distance algorithm, we are able to obtain a faster algorithm for the center distance problem:

\begin{theorem}\label{thm:k-center}
    Given $k=\Oh(1)$ straight-line programs $\G_{X_i}$ of total size $n$ generating strings $X_i$
    of total length $N>0$ and a parameter $\eps \in (0,1]$,
    an integer between $\CED(X_1,\ldots,X_k)$ and $(1+\eps)\CED(X_1,\ldots,X_k)$
    can be computed in $O\left(\eps^{-\Oh(k)}n^{k/2}N^{k/2+o(1)}\right)$ time.
\end{theorem}

The proof is given in~\cref{sec:k-ced}.
The algorithm is similar to the algorithm behind Theorem~\ref{thm:k-ed}, again using the window-respecting alignment framework.
The main difference between this algorithm and our edit distance algorithm is that it does not suffice to just compute the center distance between each tuple of windows. This is because it may be optimal to,
say, incur extra edits on the first window we use in $X_2$ to reduce the edits we use on the first window in $X_1$, provided that $X_1$ will have to incur many more edits in later windows, even though this may increase the local center distance within the first tuple of windows. 
Hence, for every tuple of windows, our DP needs to (approximately) compute all vectors $v$ such that we can align all the strings using at most $v_i$ edits to the $i$th string.

Our algorithm now needs to perform convolutions of sets of vectors instead of adding integers, and if we simply made this substitution in our algorithm for median distance, most of the work of the algorithm would be performing convolutions. To make convolutions cheaper to perform, we can ``sparsify'' the vectors $v$ we compute, by rounding them up to multiples of roughly $\epsilon D \tau / N$, where $\tau$ is the window size we use and $D$ is our guess for the center distance. This allows us to perform convolutions in time $\tilde{O}_\epsilon((N/\tau)^k)$, instead of $\tilde{O}(N^k)$, and we would need to perform $\tilde{O}_\epsilon((N/\tau)^k)$ convolutions. However, $\tau$ needs to be rather large for this to be a significant reduction in the work taken, and the time spent computing the vectors for any tuple of windows might be quite a large function of $\tau$. For example, if we use the exact algorithm of \cite{NicolasRivals05} on each of tuple of windows and use compression to bound the number of tuples of windows we need to run the exact algorithm for, we only get a bound of roughly $O(n^k \tau^{3k})$ time spent computing vectors for all tuples of windows. Optimizing for $\tau$, this gives a final runtime of roughly $O(N^{6k/5} n^{8k/5})$, far from our desired runtime. 

This motivates us to use recursion. The idea is that if $\tau$ is close to $N$, the non-recursive work per subproblem is fairly negligible. At the same time, if $\tau$ were small, then we could exactly solve the center distance problem for all tuples of windows efficiently. In one iteration of splitting strings up into windows we cannot have both properties, but we are able to show that with $\log \log N$ levels of recursion we only need a small amount of non-recursive work per subproblem while also keeping the total work spent on base cases quite small. Some additional technical work is needed to ensure the number of distinct subproblems is small while preserving the approximation ratio; we defer the details to Section~\ref{sec:k-ced}.
% In turn, our DP now needs to perform a potentially $\tilde{O}(N^k)$-time convolution of sets of vectors instead of each $O(1)$-time addition it was doing in the median edit distance setting.
% The cost of performing convolutions skews the workload of the algorithm heavily towards the time spent filling the DP table.
% Consequently, our runtime is minimized by using $N^{o(1)}$ windows of length $N^{1-o(1)}$ in each string, so that there are very few entries in the DP table to begin with. This means that compression can only shave $N^{o(1)}$ factors off our final runtime, and so we state the algorithm in the uncompressed setting only.

As an aside, note that $\min_i \sum_{i' \neq i} \ED(X_i, X_{i'})$ is a 2-approximation of the median edit distance, and similarly, $\min_i \max_{i' \neq i} \ED(X_i, X_{i'})$ is a 2-approximation of the center edit distance. 
Both can be computed using $O(k^2)$ edit distance computations on two strings. Thus, we can get a $(2+\epsilon)$-approximation for the both median and center edit distance of $k=\Oh(1)$ compressed strings via \cref{thm:edap} in time $\Ohtilde\left(n^{4/3}N^{2/3}\eps^{-1/3}\right)$.

\subsubsection*{Shift Distance of Multiple Strings}
We also consider the problem of \ComBkAlig. This can be viewed as a problem of finding the best rotations (shifts) of strings so that the shifted strings have maximum number of matching coordinates. We get tight upper and lower bounds for this problem. This problem was studied in the case of two strings previously~\cite{compressedLCSSETH,AndoniIKH13}.
\begin{theorem}\label{thm:cycShiftUB}
There is an $O(|\Sigma|N^{k-1}\lg(|\Sigma|N))$ algorithm for \ComBkAlig.
\end{theorem}

For this problem we get a tight lower bound when the strings are highly compressible. This lower bound shows that uncompressed strings have no faster algorithms than compressed strings if SETH holds.

\begin{theorem}\label{thm:cycShiftLB}
Let $a$ and $k$ be constants. If the $(a(k-1))$-OV hypothesis holds then
\ComBkAlig~requires $N^{k-1-o(1)}$ time even when the strings compress down to size $m=N^{1/a + o(1)}$ with an alphabet of size $O(1)$.
\end{theorem}

However, we do have a faster algorithm when approximation is allowed. 

\begin{theorem}\label{thm:cycShiftApprox}
There is an $O\left(|\Sigma|N^{\lceil (k-1)/\ell  \rceil}\lg(|\Sigma|N)\right)$-time algorithm to get an $\ell$-approximation of the \ComBkAlig\ for any integer $\ell\geq 2$.
\end{theorem}


==> TechnicalSummaryHammingDistance.tex <==
\subsubsection*{Hamming Distance and Beyond}
Surprisingly, the problem of computing the Hamming distance between two grammar-compressed
strings is less understood than its edit distance counterpart.
The trivial decompress-and-solve algorithm takes $\Oh(N)$ time.\footnote{Note that the Hamming distance $\HD(X,Y)$ is well defined only if the strings $X$ and $Y$ have equal lengths $N=M$.}
Abboud, Backurs, Bringman, and Künnemann~\cite{compressedLCSSETH}
presented an $\Ohtilde((n+m)^{1.41}N^{0.593})$-time algorithm, which improves upon $\Oh(N)$ for highly compressible strings.
Moreover, they gave a series of lower bounds: in particular, conditioned on the 
Strong $(2k+1)$-Sum Conjecture, $N^{1/3 + 2/(9k+3)-o(1)}$ time
is necessary for $N = \Theta(n^{3k+1})=\Theta(m^{3k+1})$.
In~\cref{sec:Hamming}, we improve upon the algorithm of~\cite{compressedLCSSETH},
achieving $\Oh(\sqrt{nmN})=\Oh((n+m)N^{0.5})$ time.

\begin{theorem}\label{thm:Hamming}
    Given a straight-line program $\G_X$ of size $n$ generating a string $X$ of length $N>0$
    and a straight-line program $\G_Y$ of size $m$ generating a string $Y$ of the same length $N$,
   the Hamming distance $\HD(X,Y)$ can be computed in $\Oh(\sqrt{nmN})$ time.
\end{theorem}

The algorithm behind \cref{thm:Hamming} is inspired by that of \cref{thm:edexact};
in particular, we use the same decompositions of $X$ and $Y$,
and we construct a counterpart of the $\DIST$ matrices for each box.
Since the Hamming distance involves substitutions only, an input vertex uniquely determines
the corresponding output vertex, so the number of distances to be computed is linear in the perimeter of the box. Consequently, precomputing the distances for all distinct boxes in $\Oh(nm\tau)$ time is rather easy.
The final dynamic-programming step also simplifies a lot: we just need to follow the main diagonal,
passing through $\Oh(\frac{N+M}{\tau})$ boxes (with a single input and a single output vertex per box).
Balancing the running times of these two steps, we obtain the $\Oh(\sqrt{nmN})$ running time.

We also observe that the same scheme allows computing various generalizations of Hamming distance to $k=\Oh(1)$
strings $X_1,\ldots,X_k$ of common length $N$ and compressed sizes $n_1,\ldots,n_k$
in $\Oh\left((n_1\cdots n_k)^{1/k}N^{1-1/k}\right)$.

In order to formulate the core of our approach as a black box (independent of any particular generalization of $\HD$),
we actually develop an algorithm that constructs a grammar-compressed representation
of a string $X$ whose $j$th character $X[j]$ is a tuple $(X_1[j],\ldots,X_k[j])$.
Then, for any function $\delta$ defined on $k$-tuples of characters,
the value $\sum_{j=1}^N \delta(X_1[j],\ldots,X_k[j])$ can be computed efficiently by processing the grammar 
generating $X$ in time proportional to the size of this grammar,
which is $\Oh\left((n_1\cdots n_k)^{1/k}N^{1-1/k}\right)$.


==> abstract.tex <==
Real-world data often comes in compressed form.
Analyzing compressed data directly (without first decompressing it) can save space and time by orders of magnitude. 
In this work, we focus on fundamental sequence comparison problems and try to quantify the gain in time complexity when the underlying data is highly compressible. 
We consider grammar compression, which unifies many practically relevant compression schemes such as the Lempel--Ziv family, dictionary methods, and others.

For two strings of total length $N$ and total compressed size $n$, it is known that the edit distance and a longest common subsequence (LCS) can be computed exactly in time $\Ohtilde(nN)$, as opposed to $O(N^2)$ for the uncompressed setting.
Moreover, this time bound is essentially optimal assuming the Strong Exponential Time Hypothesis (SETH).
Many real-world applications need to align multiple sequences simultaneously. 
Given $k$ strings, it is known that computing an LCS or a median string under the edit distance takes $\Oh(N^k)$ time and that this running time is essentially optimal under SETH.
The success in the two-strings case naturally raises the question if compression can help to reduce the running time significantly for $k \geq 3$, perhaps to $O(N^{k/2}n^{k/2})$ or, more optimistically, to $O(Nn^{k-1})$.

\begin{description}[leftmargin=0pt]
\item[Lower Bound.] Unfortunately, our first result shows that computing the LCS length or the median edit distance of $k$ strings essentially requires $\Omega(N^{k-1}n)$ time under SETH, where again $N$ and $n$ represent the total length and the total compressed size, respectively. In other words, the savings become negligible as $k$ grows. This also answers an open question of [Abboud, Backurs, Bringmann, K{\"{u}nnemann}, FOCS'17].
\end{description}

\noindent In presence of such negative results, we ask if allowing approximation can help, and we show that approximation and compression together can be surprisingly effective for both multiple and two strings.
\begin{description}[leftmargin=0pt]
\item[Upper Bounds with Approximation \& Compression.] 
We develop an $\tilde{O}(N^{k/2}n^{k/2})$-time FPTAS for the median edit distance of $k$ sequences, leading to a saving of nearly half the dimensions for highly-compressible sequences.
In comparison, no $O(N^{k-\Omega(1)})$-time PTAS is known for the median edit distance problem in the uncompressed setting.
For two strings, we obtain an $\Ohtilde(N^{2/3}n^{4/3})$-time FPTAS for edit distance; note that this running time is $o(N)$ whenever $n \ll N^{1/4}$.  Similarly, in $\Ohtilde(N^{2/3}n^{4/3})$ time, we can approximate the LCS length from below within an $\Oh(\lambda)$ factor if the LCS length is $\Theta(N/\lambda)$. In contrast, for uncompressed strings, the $\Oh(N^{2-\Omega(1)})$ time is only known to allow for an $\Oh(\lambda^3)$-approximation.

\item[Exact Upper Bounds with Compression] Building on the insight from our approximation algorithms, we also obtain some new and improved results for exact computation.
We show if edit distance between two strings is bounded by $D$, then it can be computed exactly in time $\Ohtilde(n \sqrt{ND})$. This improves upon the best known bound of $\Ohtilde(\min(nN, n+D^2))$ whenever $D \gg N^{1/3}n^{2/3}$.
As for the Hamming distance, we obtain an $\Oh(n\sqrt{N})$-time algorithm, improving upon an $\Oh(n^{1.41}N^{0.59})$-time solution of [ABBK, FOCS'17].
\end{description}

Finally, we consider the $k$-center string problem under edit distance, for which the best running time~is $O(N^{2k})$. Surprisingly, our techniques yield an $O(N^{k+o(1)})$-time FPTAS already for uncompressed strings.

==> kEditDist.tex <==

\subsubsection*{Easy $k$-Median Edit Distance lower bounds via LCS reduction}
As a first lower bound for edit distance, we can reduce from LCS to both median $k$-edit distance and center $k$-edit distance. Suppose, we are given a $k$-LCS instance with strings $S_1,\ldots,S_{k}$ all of length $M$ and let $\emptystring$ denote the empty string. It can be shown that
$$\ED(S_1,\ldots,S_{k},\underbrace{\emptystring,\ldots,\emptystring}_{(k-1)}) = Mk - \lcsf(S_1,\ldots,S_{k}).$$
This increases $k$ since we add $(k-1)$ empty strings, but it does not increase the size of the problem, or the compression size. Using the above relation, we can prove the following theorem.
%We get one lower bound from a general $k$-LCS to $k'$-Edit Distance reduction. This reduction adds $(k'-k)$ empty strings to the $k$-LCS instance. This increases $k$, but does not increase the size of the problem. This general purpose reduction may be useful in other settings as well.
%\begin{theorem}\label{thm:medianEDhardLCS}
%We are given a $k$-LCS instance with strings $S_1,\ldots,S_{k}$ all of length $M$. Let the $k$-LCS distance of these strings be $\lcsf(S_1,\ldots,S_{k})$.
%Then, let $\emptystring$ be the empty string we now relate $(2k-1)$-median edit distance to $k$-LCS. Specifically, $(2k-1)$-median edit distance on $S_1$ through $S_k$ and $k-1$ copies of the empty string and the $k$-LCS of $S_1$ through $S_k$:
%$$\ED(S_1,\ldots,S_{k},\emptystring,\ldots,\emptystring) = Mk - \lcsf(S_1,\ldots,S_{k}).$$
%\end{theorem}

\begin{theorem}
\label{thm:EditDistanceSethHard}
Given an instance of $k$-median edit distance on strings of lengths $M_1 \leq M_2 \leq \ldots \leq M_{k}$ where these strings can all be compressed into a SLP of size $m=|\sum_{i} M_i|^{\delta\pm o(1)}$ for any constant $\delta \in (0,1]$. 
Then, an algorithm for $k$-median edit distance that runs in 
$\left((M_2+1) \cdots (M_{k}+1) \cdot m  \right)^{1-\epsilon}$ time for constant $\epsilon>0$ violates SETH.
\end{theorem}

\noindent We can get a similar lower bound for center $k$-edit distance from $k$-LCS by adding a single empty string.

\begin{theorem}
\label{thm:centerFromLCS}
Given an instance of $k$-center edit distance on strings of lengths $M_1 \leq M_2 \leq \ldots \leq M_{k}$ where these strings can all be compressed into a SLP of size $m=|\sum_{i} M_i|^{\delta\pm o(1)}$ for any constant $\delta \in (0,1]$, then, an algorithm for $k$-center edit distance that runs in time 
$\left((M_2+1) \cdots (M_{k}+1) \cdot m  \right)^{1-\epsilon}$ time for constant $\epsilon>0$ violates SETH.
\end{theorem}

%We can get a similar generic lower bound for center $k$-edit distance from $k$-LCS.
%\begin{theorem}\label{thm:centerEDhardLCS}
%We are given a $k$-LCS instance with strings $S_1,\ldots,S_{k}$ all of length $M$. Let the $k$-LCS distance of these strings be $\lcsf(S_1,\ldots,S_{k})$.
%Then, let $\emptystring$ be the empty string we now relate $(k+1)$-center edit distance and $k$-LCS:
%$$\CED(S_1,\ldots,S_{k},\emptystring) \begin{cases}
%=M/2 & \text{  if }\lcsf(S_1,\ldots,S_{k})=M/2\\
%> M/2 &\text{  if }\lcsf(S_1,\ldots,S_{k})\ne M/2\\
%\end{cases}.$$
%\end{theorem}

These reductions are convenient for propagating results from $k$-LCS to $k$-Edit Distance generically. However, because they add empty strings, they don't prove hardness for some of the most commonly studied cases such as where all strings are of the same length and for median $k$-edit distance with even $k$. To get lower bounds for all $k$ and when all strings are of the same length, we use a reduction directly from SETH, instead of going through $k$-LCS.

\subsubsection*{Stronger $k$-Median Edit Distance Lower Bounds directly from SETH}
We get a lower bound for median $k$-edit distance and center $k$-edit distance over compressed strings from SETH. When $k=2$ this resolves the second open problem suggested by Abboud et al~\cite{compressedLCSSETH}. We also generalize the lower bound for all $k\geq 2$. There are many difficulties introduced by trying to get lower bounds for median $k$-edit distance when $k\geq 2$. We can use some of the ideas from the $k$-LCS reduction. Specifically, the notion of the compressed interleaved strings remains. 
%However, because $k$-edit distance allows not just deletions but also insertions and substitutions we need to change our perfect alignment gadget. 
Notably, we need to allow any choice of $\Delta_1,\ldots,\Delta_{k-1}$ offsets; however, if these offsets are more similar we have many characters that match on all but one string. For $k$-LCS we still need to delete these characters, but, in median $k$-edit distance we can simply insert a character in one string. 
%Matches on $k-1$ strings are cheaper than cases where a character matches on only $k/2$ strings. 
This creates an artificial pressure to make all the $\Delta_i$ values the same. To overcome this, we  can use some of the ideas from the recent paper that gives lower bounds for the uncompressed case for $k$-edit distance~\cite{editDistLBSeth}. There is still an issue, they build their alignment gadget with the crucial use of empty `fake gadgets'. However, we need to guarantee that $\Delta_i\in[0,n^a-1]$, and these fake gadgets allow for values of $\Delta_i$ outside of this range. 
To overcome this we incentivize a match up of the real gadgets, which then forces a restriction on valid $\Delta_i$ values. 

Specifically, we need to add a gadget, which we call a selector gadget. This gadget causes characters lined up inside it to have a low edit distance if they all match, and otherwise have a higher edit distance that is unchanged by exactly how well they match. The selector gadget looks like this:
$SCSG_i(c) = \%^{ix} c^y \%^{(k-i)x}.$
We have gadgets $SCSG_1(c_1),\ldots,SCSG_k(c_k)$ such that we can either try to match the characters $c_i$, or try to line up the $\%$ characters. If we line up the $\%$ characters, the edit distance is $ky$. If we line up the $c_i$ characters and they all match ($c_i=c_j~ \forall i,j$ ), the edit distance is $xk^2/4$ if $k$ is even and $x(k^2-1)/4$ if $k$ is odd. If the characters don't match the edit distance is at least $xk^2/4+y$ if $k$ is even and $x(k^2-1)/4+y$ if $k$ is odd. Consider the case of $k$ even, we can choose integer values of $x$ and $y$ such that
$xk^2/4 < yk \leq xk^2/4+y.$
By doing so, if all the characters match, then the median $k$-edit distance is $xk^2/4$, otherwise it is $yk$.
In some sense this gadget is causing characters to act like they do in $k$-LCS, where only a match across all strings gives us a benefit. Using these selector gadgets and ideas from the edit distance and LCS lower bounds, we get a lower bounds for both median $k$-edit distance and center $k$-edit distance from SETH. 

\begin{theorem}\label{thm:editDistanceLowerBoundFromSETH}
If the $k'$-OV hypothesis is true for all constants $k'$, then for all constant $\epsilon \in (0,1]$ grammar-compressed $k$-median edit distance requires $\left(M^{k-1}m\right)^{1-o(1)}$ time when the alphabet size is $|\Sigma|=\Theta(k)$ and $m=M^{\epsilon \pm o(1)}$. Here, $M$ and $m$ denote the total uncompressed and compressed length of the $k$ input strings respectively.
%Let $b$ be a positive integer $b\geq 1$.
%If for positive integers $a$, $b$, and $k$ we have that $(bk+a(k-1))$-OV requires $n^{bk+a(k-1)-o(1)}$ time then SLP compressed $k-$edit distance requires $\left(M^{k-1}m\right)^{1-o(1)}$ time when $m = M^{b/(a+b)}$ and there is an alphabet of size $|\Sigma|=\Theta(k)$. Recall that $M$ is the length of the $k$ input strings to SLP compressed $k-$edit distance  and $m$ is the size of the SLP compression.
\end{theorem}

The lower bound for median $k$-edit distance immediately implies a lower bound for center $k$-edit distance following~\cite{editDistLBSeth}. %However, $k$-center is a harder problem, making this less tight than the median $k$-edit distance result. 

\begin{theorem}\label{thm:centerEditDistanceAllSameLength}
We are given $k$ strings of length $M$ with a SLP of size $m$. The center $k$-edit distance problem on these strings requires $\left(M^{k-1}m \right)^{1-o(1)}$ time if SETH is true. 
\end{theorem}

Given these lower bounds for the case of compressed $k$-LCS, median $k$-edit distance and center $k$-edit distance, we want to consider not just compression but also approximation. 

==> mediandistance-deferred.tex <==
\section{Deferred Proofs from Section~\ref{sec:k-ed}}\label{sec:k-ed-deferred}

\subsection{Proof of Lemma~\ref{lemma:lowskew}}

\begin{proof}

We partition $X_1$ into substrings of length $\tau$, $\{X_{1,j}\}_{j \in [J]}$. $X^*$ can be partitioned into substrings  $\{\tilde{X}^*_j\}_{j \in [J]}$ such that $\ED(X_1, X^*) = \sum_{j \in [J]} \ED(X_{1, j}, \tilde{X}^*_j)$.

First, we will ``realign'' $X_1$ and $X^*$ to ensure no $\tilde{X}^*_j$ is much larger than $X_{1, j}$. Call a contiguous subsequence of $[J]$, $\subseq{j}{j'}:= \{j, j+1, \ldots j'\}$, ``skewed'' if $\sum_{m \in \subseq{j}{j'}} |X_{1, m}| < \frac{\epsilon}{2} \sum_{m \in \subseq{j}{j'}} |\tilde{X}^*_m|$. Let us take a ``maximal'' set $S$ of disjoint skewed contiguous subsequences, i.e. a set $S$ such that (i) all the subsequences in $S$ are disjoint (ii) for every contiguous subsequence $s$ in $S$, there is no skewed contiguous subsequence $s'$ such that $s \subset s'$ and (iii) there is no skewed contiguous subsequence that is not in $S$ but also is completely disjoint from every element of $S$.

For each skewed contiguous subsequence $\subseq{j}{j'}$ in $S$, note that $j'+1$ does not appear in any element of $S$ (otherwise, $\subseq{j}{j'}$ and this element can be combined to form a longer skewed contiguous subsequence, violating (ii)), and $\subseq{j}{j'+1}$ is not skewed (again, $\subseq{j}{j'+1}$ being skewed would violate (ii) since $\subseq{j}{j'} \subset \subseq{j}{j'+1}$). Take $S$ and replace each $\subseq{j}{j'}$ with $\subseq{j}{j'+1}$ to get $S'$. For each $\subseq{j}{j'+1} \in S'$, we have:

\begin{equation}\label{eq:lengthbound}
\frac{\epsilon}{2} \sum_{m \in \subseq{j}{j'+1}} |\tilde{X}^*_m| \leq \sum_{m \in \subseq{j}{j'+1}} |X_{1, m}| \leq 2 \sum_{m \in \subseq{j}{j'}} |X_{1, m}|< \epsilon \sum_{m \in \subseq{j}{j'+1}} |\tilde{X}^*_m|.
\end{equation}

The right hand side of~\eqref{eq:lengthbound} implies:

\[\ED(\bigcirc_{m  \in \subseq{j}{j'+1}} X_{1, m}, \bigcirc_{m  \in \subseq{j}{j'+1}} \tilde{X}^*_m) \geq (1 - \epsilon) |\bigcirc_{m  \in \subseq{j}{j'+1}} \tilde{X}^*_m|.\]

It also implies that for any partition of $\bigcirc_{m  \in \subseq{j}{j'+1}} \tilde{X}^*_m$ into substrings $\{X^*_m\}_{m  \in \subseq{j}{j'+1}}$, we have:

\[\sum_{m  \in \subseq{j}{j'+1}} \ED(X_{1, m}, X^*_m) \leq (1+\epsilon) |\bigcirc_{m  \in \subseq{j}{j'+1}} \tilde{X}^*_m|.\]

And so if $\epsilon$ is sufficiently small:

\[\sum_{m\in \cup_{e \in S'} e} \ED(X_{1,m}, X^*_m) \leq \frac{1+\epsilon}{1-\epsilon}\sum_{m\in \cup_{e \in S'} e} \ED(X_{1,m}, \tilde{X}^*_m) \leq (1+3\epsilon)\sum_{m\in \cup_{e \in S'} e} \ED(X_{1,m}, \tilde{X}^*_m)\]

In particular, because of the left hand side of~\eqref{eq:lengthbound}, we can choose the partition of $\bigcirc_{m  \in \subseq{j}{j'+1}} \tilde{X}^*_m$ that splits it into substrings $\{X^*_m\}_{m  \in \subseq{j}{j'+1}}$, each of length at most $2\tau/\epsilon$. 

Now if we set $X^*_m = \tilde{X}^*_m$ for any $m$ not in a subsequence in $S'$, we trivially have:

\[\sum_{m\notin \cup_{e \in S'} e} \ED(X_{1,m}, X^*_m) \leq \sum_{m\notin \cup_{e \in S'} e} \ED(X_{1,m}, \tilde{X}^*_m)\]

And also $X^*_{m} \leq 2\tau/\epsilon$ for all such $m$ (otherwise, $m$ should appear in some subsequence in $S'$ by condition (iii)). So we've found a partition of $X^*$ into substrings $\{X^*_j\}_{j \in [J]}$ such that $|X^*_j| \leq \frac{1}{\epsilon}|X_{1,j}|$ for all $j$, and:

\[\sum_{j \in [J]} \ED(X_{1,j}, X^*_j) \leq (1+3\epsilon)\sum_{j \in [J]} \ED(X_{1,j}, \tilde{X}^*_j).\]

Now, we will use this partition to determine $\{X_{i,j}\}_{i > 1, j \in [J]}$. For each $i$, $X_i$ can be partitioned into substrings $X'_{i, j}$ such that $\ED(X_i, X^*) = \sum_{j \in [J]} \ED(X'_{i,j}, X^*_j)$. If $|X'_{i,j}| \leq 2\tau/\epsilon^2$, we set $X_{i,j} = X'_{i,j}$. If any $X'_{i,j}$ has length larger than $2\tau/\epsilon^2 > |X^*_j| / \epsilon$, then $\ED(X'_{i,j}, X^*_j) \geq (1-\epsilon)|X'_{i,j}|$. On the other hand:

\[\ED(\gamma, X^*_j) + |X'_{i,j}| \leq (1+\epsilon)|X'_{i,j}| \leq \frac{1+\epsilon}{1-\epsilon} \ED(X'_{i,j}, X^*_j) \leq (1+3\epsilon) \ED(X'_{i,j}, X^*_j) \]
for the empty string $\gamma$. So we can now choose $X_{i,j}$ to be any empty substring of $X'_{i,j}$. These choices of $X_{i,j}$ give the properties of the lemma, completing the proof.
\end{proof}

\subsection{Proof of~\cref{lemma:ked-window}}

\begin{proof}
The first inequality follows because for any $f$, there is an alignment that for all $j$ exactly aligns $W_{1,j}$ with the windows in $f(W_{i,j})$ at cost at most $\ED(f(W_{i,j})$, and uses $\sum_i r_i(f)$ deletions to handle the remaining characters in each string. 

Next, we show that there exists $f \in \mathcal{F}$ such that $\ED(f) \leq (1+\epsilon k) \ED(X_1, X_2, \ldots X_k)$. Let us take the substrings $X_{i, j}$ given by Lemma~\ref{lemma:lowskew}. Note that $W_{1, j} = X_{1, j}$.

If $|X_{i, j}| \leq \epsilon \ED(W_{1, j}, X_{2, j} \ldots X_{k , j}) + 3(\sigma-1)$, let $W_{i,j}$ be the empty window ``starting'' at index $\nd(W_{i, j-1})+1$, or if $j = 1$, at index 1. Then we have $|X_{i, j}| - |W_{i, j}| \leq \epsilon \ED(W_{1, j}, X_{2, j} \ldots X_{k , j}) + 3(\sigma-1)$.

Otherwise, let $W_{i, j}$ be the longest window $W_{i, \Delta, p}$ that is a substring of $X_{i, j}$. Note that $|X_{i, j}|$ and $|W_{1, j}|$ differ by at most $\ED(W_{1, j}, X_{2, j} \ldots X_{k , j})$ and $|W_{i, j}| \leq 2\tau/\epsilon^2$ for all $i, j$. If $\epsilon$ is a sufficiently small constant, this implies there is a choice of $W_{i, j}$ such that $|X_{i, j}| - |W_{i, j}| \leq \epsilon \ED(W_{1, j}, X_{2, j} \ldots X_{k , j}) + 3(\sigma-1)$. We can identify $W_{i,j}$ as follows: Take $X_{i,j}$ and delete at most $\sigma - 1$ characters from the beginning until it starts at $p\sigma + 1$ for some integer $p$ to get $\tilde{X}_{i,j}$. We have $|X_{i, j}| - |\tilde{X}_{i, j}| \leq \sigma - 1$, and so $|\tilde{X}_{i, j}|$ and $|W_{1, j}|$ differ by at most $\ED(W_{1, j}, X_{2, j} \ldots X_{k , j}) + (\sigma - 1)$ characters. Choose $\Delta$ such that $\frac{1}{1+\epsilon} (\ED(W_{1, j}, X_{2, j} \ldots X_{k , j}) + (\sigma - 1)) \leq \Delta \leq \ED(W_{1, j}, X_{2, j} \ldots X_{k , j}) + (\sigma - 1)$. $W_{i, \Delta, p}$ is a prefix of $\tilde{X}_{i,j}$ containing all but at most the last $\epsilon (\ED(W_{1, j}, X_{2, j} \ldots X_{k , j}) + (\sigma - 1)) + (\sigma - 1)$ characters of $\tilde{X}_{i,j}$. In turn, if $\epsilon$ is sufficiently small we have $|X_{i, j}| - |W_{i, j}| \leq \epsilon \ED(W_{1, j}, X_{2, j} \ldots X_{k , j}) + 3(\sigma-1)$.

In turn, by triangle inequality and since $\sigma - 1 \leq \epsilon k D \tau / |X_1|$:

\[\ED(W_{1, j}, W_{2, j} \ldots W_{k, j}) \leq (1 + \epsilon k) \ED(W_{1, j}, X_{2, j} \ldots X_{k, j}) + 3\epsilon k D \tau/|X_1|.\]

We now choose $f(W_{1, j}) = (W_{1, j}, W_{2, j} \ldots W_{k, j})$. We also have that the number of characters $f$ does not align within $X_{2, j}, X_{3, j} \ldots X_{k, j}$ is at most $\epsilon k\ED(W_{1, j}, X_{2, j} \ldots X_{k , j}) + 3\epsilon k D \tau/|X_1|$.

Putting it all together and using Lemma~\ref{lemma:lowskew} we get:
\begin{align*}
\ED(f) := &\sum_{j\in [J]} \ED(f(W_{1, j})) + \sum_i r_i (f)\\
\leq &
(1 + \epsilon k) \sum_j \ED(W_{1, j}, X_{2, j} \ldots X_{k , j}) +\frac{|X_1|}{\tau} \cdot \frac{3 \epsilon k D \tau}{|X_1|} \\
&\qquad+ \epsilon k \sum_j \ED(W_{1, j}, X_{2, j} \ldots X_{k , j})+\frac{|X_1|}{\tau} \cdot \frac{3 \epsilon k D \tau}{|X_1|} + \sum_i (|X_i| - \sum_{j \in [J]} |X_{i, j}|)\\
\leq &
(1+2 \epsilon k) \sum_j \ED(X_{1,j}, X_{2,j}, \ldots X_{k,j}) + 6 \epsilon k \ED(X_1, X_2, \ldots, X_k) + \sum_i (|X_i| - \sum_{j \in [J]} |X_{i, j}|)\\
\leq &
 (1+13\epsilon k) \ED(X_1, X_2, \ldots X_k).
\end{align*}
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:lz77-repetition}}

\begin{proof}
If $\delta_{\max} \geq \tau$, we can trivially choose $S$ that only contains the empty substring, and the data structure just returns the empty substring for any query. So assume $\delta_{\max} < \tau$.

Given that $\G$ has size $n$, the optimal LZ77 factorization of $X$ has size at most $n$ \cite{Rytter2003}. We will first show the existence of $S$ for any $X$ that has an LZ77 factorization of size at most $n$. For brevity, we will not go into the details of LZ77 factorization here. The key property we need is that a string $X$ that has a LZ77 factorization of size $n$ can be written as $X_1 \circ X_2 \circ X_3$, where $X_1$ is a string with LZ77 factorization of size $n-1$, $X_2$ is a substring of $X_1$, and $X_3$ is a single character. Moreover, the factorization gives the location of $X_2$ in $X_1$. 

Inductively, suppose we have constructed $S$, a set of at most $3 (n-1) \tau / \delta_{\max}$ substrings that has the desired properties for $X_1$. For all ``good'' indices $i <  |X_2| - \tau$, the length $\tau$ substring starting at the $i$th character in $X_2$ is fully contained in $X_2$, and thus is a substring in $X_1$. This leaves at most $\tau + 1$ ``bad'' indices where the length $\tau$ substring starting at these indices may not have a nearby string in $S$: those starting at indices $|X_1| - \tau + 1$ to $|X_1|$ of $X_1$, and the substring starting at index $|X_2| - \tau + 2$ of $X_2$. Consider the length $\tau$ substring starting at every $(\delta_{\max}/2)$-th position in indices $|X_1| = \tau + 1$ to $|X_1|$ of $X_1$, as well as the length $\tau$ substring starting at index $|X_2| - \tau + 2$ of $X_2$. This set of strings has size at most $2 \tau/\delta_{\max} + 1 \leq 3 \tau/\delta_{\max}$, and every length $\tau$ substring starting at a bad index is within edit distance $\delta_{\max}$ of some string in this set. So adding these strings to $S$ gives that $S$ now has size at most $3 n \tau / \delta_{\max}$ and has the desired properties.


For an efficient implementation of this procedure, we can compute the optimal LZ77 factorization in $O(|X|)$ time \cite{RodehPE81}. Given the LZ77 factorization, we decompose $X$ into $X_1 \circ X_2 \circ X_3$ as before, and recursively compute an array $A$ for indices in $\subseq{1}{|X_1|-\tau+1}$ and set $B$ with the following property: the length $\tau$ substrings starting at indices $i$ and $A[i]$ are within edit distance $\delta_{\max}$, and $A$ has at most $3(n-1)\tau/\delta_{\max}$ distinct values, which are exactly the values in $B$. 

Since the LZ77 factorization gives us the position of $X_2$ in $X_1$, we can fill in $A$ for the ``good'' indices in $X_2$ in time linear in the number of good indices. We can also fill in the values of $A$ for the bad indices, in time linear in the number of bad indices, and add these values to $B$. Overall, the algorithm takes linear time to compute $A, B$. $A$ now serves as the desired efficient data structure, and $B$ as our implicit representation of $S$.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:k-lms}}

\begin{proof}
Given $X_1, X_2, \ldots X_k$, let $\texttt{Slide}_{d_2, d_3, \ldots d_k}(j) = \max\{q: X_1[j\dd q] = X_2[j+d_2\dd q+d_2] = X_3[j+d_3\dd q+d_3]= \ldots =X_k[j+d_k\dd q+d_k]\}$. We can rewrite $\texttt{Slide}_{d_2, d_3, \ldots d_k}(j)$ as $\min_{i \in \{2, 3, \ldots, k\}} \max\{q : X_1[j\dd j+q] = X_i[j+d_i\dd q+d_i]\}$. Section 2.3 of \cite{LMS98} shows that we can compute $\max\{q : X_1[j\dd j+q] = X_i[j+d_i;q+d_i]\}$ for any $i, j, d_i$ in $O(1)$ time after $O(|X_1|+|X_i|)$ preprocessing time. So we can compute $\texttt{Slide}_{d_2, d_3, \ldots d_k}(i)$ in $O(1)$ time after $O(\sum_i |X_i|)$ preprocessing time (recall that $k = O(1)$).

Let $L^{h}(d_2, d_3, \ldots d_k)$ be the largest value of $j$ such that $\ED(X_1[1\dd j], X_2[1\dd j+d_2], X_3[1\dd j+d_3], \ldots, X_k[1\dd j+d_k]) \leq h$. We have the following recurrence relation:

\[L^{h}(d_2, d_3 \ldots, d_k) = \texttt{Slide}\left(\max \left.
\begin{cases}
L^{h-1}(d_2+1, d_3+1 \ldots, d_k+1)\\
\max_i L^{h-1}(d_2, d_3, \ldots, d_i - 1, \ldots, d_k)\\
\max_{e \in \{0, 1\}^k} L^{h-w}(d_2 - e_2 + e_1, d_3 - e_2 + e_1, \ldots, d_k - e_k + e_1)\\
\qquad \text{ for }w = \min_{i:e_i = 1} |\{j \neq i: X_i[x_i] \neq X_j[x_j] \lor e_j = 0\}|
\end{cases}
\right\}
\right)
\]

The first case considers deleting from $X_1$, the second case considers deleting a character from any of $X_2, X_3, \ldots X_k$, and the third case considers inserting characters into some subset of the strings (for which $e_i = 0$), and then matching the inserted characters with a character in the remaining strings (for which $e_i = 1$), such that we use at most $w$ insertions or substitutions.

Each $L^h(\cdot)$ only depends on $O(1)$ other values, and so we can compute each value in $O(1)$ time. In turn, we can compute the values $L^h(d_2, d_3, \ldots d_k)$ for all $0 \leq h \leq d, 0 \leq d_2 + d_3 + \ldots + d_k \leq d$ in $O(d^k)$ time. Our output for the edit distance is the smallest $h$ such that $L^h(|X_2|-|X_1|, |X_3|-|X_1|, \ldots, |X_k|-|X_1|) \geq |X_1|$, or $\infty$ if $L^d(|X_2|-|X_1|, |X_3|-|X_1|, \ldots, |X_k|-|X_1|) < |X_1|$.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:k-ed-approx}}

\begin{proof}
Consider any window-respecting alignment for which $f(W_{1,j}) = (W_{1,j}, W_{2,j}, \ldots, W_{k,j})$. If $\\ \ED(W_{1,j}, W_{2,j}, \ldots, W_{k,j}) > 0$, let $d_j$ be the smallest value in $\mathcal{D}$ such that $d_j \geq \ED(W_{1,j}, W_{2,j}, \ldots, W_{k,j}) + \epsilon k d_j$. By \cref{lemma:lz77-repetition}, for every $j$ and if $\epsilon$ is sufficiently small, by triangle inequality we have:

\begin{align*}
\ED(W_{1,j},W_{2,j}, \ldots, W_{k,j}) &\leq [\tilde{\ED}(\texttt{shift}_{d_j}(W_{1,j}),\texttt{shift}_{d_j}(W_{2,j}), \ldots, \texttt{shift}_{d_j}(W_{k,j}))]  + \epsilon k d_j \\
&\leq \ED(W_{1,j},W_{2,j}, \ldots, W_{k,j}) + 2 \epsilon k d_j\\
&\leq (1 + 5 \epsilon k)\ED(W_{1,j},W_{2,j}, \ldots, W_{k,j}).\\
\end{align*}

The first inequality implies that any path through the DP table for $c$ has total cost at least that of some window-respecting alignment, which by Lemma~\ref{lemma:ked-window} gives the first inequality in the lemma statement. The second inequality implies that for the best window-respecting alignment, there is a path through the DP table such that the cost of the path through the DP table is no more than $(1+5\epsilon)$ times the cost of the window-respecting alignment. Furthermore, this path only goes through points in the DP table such that $|x_i - x_1| \leq 4D$ for all $i$, i.e. is considered by \textsc{$k$-ED-Alg}. Combined with Lemma~\ref{lemma:ked-window} this gives the second inequality in the lemma statement if $\epsilon$ is sufficiently small.
\end{proof}

==> old-prelim.tex <==
\subsection{Similarity Measures}
%\agnote{I changed $S$ and $T$ to $X$ and $Y$ and some instances of $X'$ to $X^*$, feel free to revert}\tknote{I support the change.} ++
The Hamming distance $\HD(X,Y)$ of two strings $X,Y\in \Sigma^N$ of the same length is defined as 
the number of mismatches between $X$ and $Y$, that is $\HD(X,Y)=|\{i\in [1\dd N] : X[i]\ne Y[i]\}|$.

The edit distance $\ED(X,Y)$ of two strings $X,Y\in \Sigma^*$ is defined as the minimum number 
of character insertions, deletions, and substitutions needed to transform $X$ into $Y$.

A string $X\in \Sigma^M$ is a \emph{subsequence} of a string $Y\in \Sigma^N$
if there exists an increasing sequence $(i_1,\ldots,i_M)$ of positions in $X$
such that $X[j]=Y[i_j]$ for all $j\in [1\dd M]$. 
We write $\LCS(X_1,\ldots,X_k)$ to denote the maximum
length of a common subsequence of the strings $X_1,\ldots,X_k$.

\begin{definition}
The (median) edit distance $\ED(X_1,\ldots,X_k)$ of $k$ strings $X_1,\ldots,X_k$ is the minimum total number of edits (insertions, deletions, and substitutions) needed to make all strings $X_i$ equal some string $X^*$.
\end{definition}
Note that $\ED(X_1,\ldots,X_k) = \min_{X'} \sum_{i=1}^k \ED(X_i,X')$.

\begin{definition}
The center (edit) distance $\CED(X_1,\ldots,X_k)$ of $k$ strings $X_1,\ldots,X_k$ is the smallest $D$ such that there exists a string $X^*$ for which $\ED(X_i, X^*) \leq D$ for all $i$.
\end{definition}
Note that $\CED(X_1,\ldots,X_k) = \min_{X'} \max_{i=1}^k \ED(X_i,X')$.

\begin{definition}
The deletion distance $\ID(X_1,\ldots,X_k)$ of $k$ strings is the minimum total number of character deletions needed to make all strings $X_i$ equal some string $X^*$.
\end{definition}

We can also define the $k$-LCS of strings.

\begin{definition}
The $k$-LCS, $\LCS(X_1,\ldots,X_k)$, of $k$ strings is the maximum size of the string $|X^*|$ such that $X^*$ can be generated by deleting characters from each $X_i$. 

Note that $\sum_{i=1}^k |X_k| = k\cdot \LCS(X_1,\ldots,X_k) + \ID(X_1,\ldots,X_k)$. The LCS and deletion distance are a pair. 
\end{definition}

Next we will define \ComBkAlig. This problem has been studied previously in the case of $k=2$  \cite{AndoniIKH13,compressedLCSSETH}.

\begin{definition}[\ComBkAlig~(\CBKA)]
We are given $k$ strings as input: $X_1, \ldots, X_k$. For convenience of notation let $X_j[i]$ when $i \notin [0,n-1]$ refer to $X_j[i']$ where $i' \in [0,n-1]$ and $i' \equiv i \mod n$ (so we let indices ``wrap around''). 

Let $\hat{\Delta} = max(\Delta_1, \ldots, \Delta_{k-1})$. And let $[[\cdot]]$ be an operator that turns $True$ to a $1$ and $False$ to a $0$.
$$\CBKA(X_1,\ldots, X_k) = max_{\Delta_1, \ldots, \Delta_{k-1} \in [0,N-1]} \left( \sum_{i=1}^{N} {\biggl [\biggl[}X_1[i+\Delta_1]=X_2[i+\Delta_2]=\ldots = X_{k-1}[i+\Delta_{k-1}]=X_k[i] {\biggr ] \biggr]} \right)$$
\end{definition}
